SCExAO and Keck Direct Imaging Discovery of a Low-Mass Companion Around the Accelerating F5 Star HIP 5319

We present the direct imaging discovery of a low-mass companion to the nearby accelerating F star, HIP 5319, using SCExAO coupled with the CHARIS, VAMPIRES, and MEC instruments in addition to Keck/NIRC2 imaging. CHARIS $JHK$ (1.1-2.4 $\mu$m) spectroscopic data combined with VAMPIRES 750 nm, MEC $Y$, and NIRC2 $L_{\rm p}$ photometry is best matched by an M3--M7 object with an effective temperature of T=3200 K and surface gravity log($g$)=5.5. Using the relative astrometry for HIP 5319 B from CHARIS and NIRC2 and absolute astrometry for the primary from $Gaia$ and $Hipparcos$ and adopting a log-normal prior assumption for the companion mass, we measure a dynamical mass for HIP 5319 B of $31^{+35}_{-11}M_{\rm J}$, a semimajor axis of $18.6^{+10}_{-4.1}$ au, an inclination of $69.4^{+5.6}_{-15}$ degrees, and an eccentricity of $0.42^{+0.39}_{-0.29}$. However, using an alternate prior for our dynamical model yields a much higher mass of 128$^{+127}_{-88}M_{\rm J}$. Using data taken with the LCOGT NRES instrument we also show that the primary HIP 5319 A is a single star in contrast to previous characterizations of the system as a spectroscopic binary. This work underscores the importance of assumed priors in dynamical models for companions detected with imaging and astrometry and the need to have an updated inventory of system measurements.

==> Hip 5319 B Discovery Paper/oldtext.tex <==

--old

Over the past two decades direct imaging detections of exoplanets around young, nearby stars have increased with facility adaptive optics (AO) systems and now extreme adaptive optics systems \citep{Marois2008, Marois2010, Kuzuhara2013, Currie2015, Macintosh2015,Chauvin2017,Keppler2018,Currie2022a}.
%(\citet{Marois2008, Marois2010}, \citet{Kuzuhara2013}, \citet{Currie2013, Currie2015, Currie2020}, \citet{Macintosh2015}, \citet{Chauvin2017}, \citet{Keppler2018}). 
The majority of these detections have been of companions at separations greater than $\rho\sim0\farcs{}4$ and correspond to separations of 10-150 au from their host stars \citep[][]{Nielsen2019,Vigan2021,Currie2022b}. 

More recently, second generation extreme AO systems such as the Subaru Coronagraphic Extreme Adaptive Optics system \citep[SCExAO;][]{Jovanovich2015b, Ahn2021} and the Magellan Extreme Adaptive Optics system \citep[MagAO-X;][]{Males2020} have enabled deeper contrasts at separations less than $\rho\lesssim0\farcs{}4$. These deeper contrasts - in conjunction with noise-reducing techniques such as Stochastic Speckle Discrimination \citep[SSD;][]{Walter2019} and Angular, Spectral, and Reference Differential Imaging \citep[ADI, SDI, RDI;][]{Marois2006, Marois2000, Ruane2019} - have led to the discovery of companions with orbital radii less than 10 au \citep[][]{Chilcote2021, Steiger2021}. By continuing to drive to deeper contrasts at narrower separations we will be able to directly image companions with orbits closer to their host stars and around host stars at greater distances from earth.

%The challenges of reaching sufficient contrasts to image young, bright exoplanets is one of the chief reasons for the low yield of blind direct imaging surveys.
\textbf{The low occurrence rates of planets which can be detected via direct imaging at contrasts achievable by current instruments and extreme AO systems} is one of the chief reasons for the low yield of blind direct imaging surveys. Fortunately the \textit{Hipparcos-Gaia Catalog of Accelerations} \citep[HGCA;][]{BrandtHGCA2021} combines absolute astrometry from the Hipparcos and \textit{Gaia} missions \citep[][]{GaiaMission}, which allows a more targeted search of nearby stars that have astrometric accelerations that suggest the presence of yet-undiscovered companions. Direct imaging surveys that target these stars with significant astrometric acceleration have already yielded discoveries of companions on solar-system scales and have also enabled a better ability to characterize them (\citet{Calissendorff2018, Fontanive2019, Currie2020, Currie2021, Bowler2021, Chilcote2021, Steiger2021, Brandt2019, Brandt2021, Kuzuhara2022,Currie2022c}). \citep{Currie2022c}

\textcolor{red}{As astrometry-selected direct imaging programs become more prevalent so too will the discovery of previously undetected, uncharacterized companions. When characterizing the planets, one may use code such as \texttt{orvara} \citep[][]{Brandt2021} to fit for orbital parameters of the system such as the masses of the primary star and any existing companions as well as the eccentricity, semimajor axis, and inclination of the companion's orbit. In cases with significant coverage of a companion's orbit, archival radial velocity, astrometry for the primary, or a combination of the three, the user may be able to use the out-of-the-box priors from dynamical orbit fitting codes and achieve accurate estimates of the orbital parameters of the system without digging into the underlying assumptions used by the code. However, for systems which have not been frequently targeted and do not have archival data as such the data may not be extremely constraining for determining the parameters of system. In this paper we explore how different assumptions that go into fitting for system parameters may affect the interpretation of the results which may be as significant as the characterization of a substellar companion as a low-mass star or vise versa.}

Here we report the direct imaging discovery of HIP 5319 B, a low mass, candidate substellar companion around the F-type star HIP 5319 A using SCExAO coupled with the MKID Exoplanet Camera \citep[MEC;][]{Walter2020}, the Visible Aperture Masking Polarimetric Imager for Resolved Exoplanetary Structures \citep[VAMPIRES;][]{Norris2015}, the Coronagraphic High Angular Resolution Imaging Spectrograph \citep[CHARIS;][]{Groff2016}, and the NIRC2 camera on Keck. 


---


HIP 5319 ($^{\star}$78 Psc) is an F5IV spectral class star \citep{BoroSaikia2018} at $d=$42.93$\pm$0.06 pc (\citet{GaiaMission}, \citet{GaiaDR2}).

% The \textit{Hipparcos-Gaia} Catalog of Accelerations reports a $\chi^{2}=$171.04: evidence of a 12.9-$\sigma$ significant acceleration of the primary with 2 degrees of freedom \citep[][]{BrandtHGCA2021}). \textbf{The statistically significant acceleration of HIP 5319 is suggestive of the presence of a previously unseen low-mass companion. Therefore we chose to observe this target in an attempt to uncover any previously unimaged low-mass companions around this accelerating star, following a similar method of target selection as in \citet{Currie2020} and \citet{Steiger2021}.}

It has previously been identified as an RS CVn binary star by \citet{Fleming1989}, who measured a projected rotation rate of \textit{v}sin(\textit{i})=68$\pm$20.5 km/s and x-ray luminosity of $L_{x}=9.2\pm3.7\times10^{28}$ erg/s. RS CVn binaries typically have \textbf{orbital} periods less than 14 days, show high levels of chromospheric activity \textbf{via strong emission in Calcium II H and K lines, and have a hotter component of spectral type F or G \citep[][]{Montesinos1988}}. Both variation in the reported rotation rate and high chromospheric activity have been reported for this star, the latter via \textbf{Ca II} H $\&$ K lines \citet{BoroSaikia2018} measured log($R^\prime_{HK}$)= $-$4.016\textbf{, which tracks the strength of the emission at the cores of the 2 lines}. Multiple sources have reported \textit{v}sin(\textit{i}) values with significant scatter: 125 km/s \citep[][]{Danziger1972}, 68$\pm$20.5 km/s \citep[][]{Fleming1989}, 36.4$\pm$4.8 km/s \citep[][]{deMedeiros1999}, 35 km/s \citep[][]{Nordstrom2004}, and 41.5 km/s (\citet{Glebocki2005}, \citet{Glebocki2005Catalog}).

\textcolor{red}{The extreme chromospheric activity measured by \citet{BoroSaikia2018} is evidence for the extreme youth of HIP 5319. The chromospheric index of log($R^\prime_{HK}$)=-4.016 easily exceeds chromospheric activity values from stars in the Pleiades and Hyades associations and is comparable or higher to the stars in the Scorpius-Centaurus (Sco-Cen) association \citep[][]{MamajekHillenbrand2008, Pecaut2013}. Its Hertzsprung-Russel diagram position in \textit{Gaia} color-magnitude space ($M_{G}$ vs $G_{BP}-G_{RP}$=2.97, 0.54) lies between the Pleiades and Hyades, which is consistent with either a main sequence star between 115 and $\sim$800 Myr or a pre-main sequence star much younger than the Pleiades.}

In contrast to this characterization of HIP 5319 as a \textcolor{red}{young,} short period binary, the Gaia Early Data Release 3 \citep[Gaia eDR3;][]{GaiaEDR3} reports that HIP 5319 is well fit by a 5-parameter single star solution whose Renormalized Unit Weight Error (RUWE) is 1.01, \textbf{ruling out most stellar companions with a period between of P$\lesssim$10 days}.
%(Timothy Brandt, private communication).

\textcolor{red}{The fractional X-ray luminosity of the star is log($L_{x}$/$L_{bol}$)$\sim$-4.9, almost two orders of magnitude less than a typical pre-main sequence star, which would have values log($R^\prime_{HK}$)$\sim$-4.0 and log($L_{x}$/$L_{bol}$)$\sim$-3.2 for the chromospheric activity and fractional X-ray luminosity, respectively. This mix of chromospheric and coronal activity is therefore atypical compared to other young, active stars. The star also does not appear to be near any other stars or known associations that are $\lesssim$100 Myr. Several authors have estimate the age of the star using isochrones and have found values of $1.6^{+0.3}_{-0.4}$ Gyr \citep[][]{Holmberg2009} and 1.07-1.23 Gyr using Padova and BASTI models \citep[][]{Casagrande2011}, lending credence to its identification as an older, single star.}

\textcolor{red}{Ultimately, the two conflicting identifications of the HIP 5319 primary as either a young, chromospherically active binary or an older single star that lacks Calcium II HK emission will have significant implication on the understanding of the stellar system and interpretation of any of its companions' properties. If there is not significant HK emission and little evidence of binarity then the higher age estimate is likely the correct one, which will anchor the interpretation of its companion.} In addition to performing a direct imaging search for such a binary companion, a spectroscopic \textbf{study} of the primary with a high resolution spectrograph is necessary to disentangle the possible identities of the star and settle on the correct interpretation. This will be discussed further in sections \ref{sub:primary_single_star} and \ref{sub:ca_hk}.

More recently, HIP 5319 was observed by the Transiting Exoplanet Survey Satellite \citep[TESS;][]{TESS_Mission} and has 2-minute cadence photometry for one sector. This observation may be too short to show spots reliably, but it does show pulsations with a period of just less than 1 day\footnote{Accessed via \url{https://mast.stsci.edu/portal/Mashup/Clients/Mast/Portal.html}}. It was also observed once by the International Ultraviolet Explorer (IUE) during IUE Program ID: CB401 \citep[Stellar Chromospheres;][]{Blanco1982}. In the spectrum from IUE\footnote{Accessed via \url{https://archive.stsci.edu/iue/obtaining.html}}, HIP 5319 A shows strong emission from the Lyman $\alpha$ line. These two data points show signs that the primary might be chromospherically active, though follow up observation is required to determine the nature of this activity.

The \textit{Hipparcos-Gaia} Catalog of Accelerations reports a $\chi^{2}=$171.04: evidence of a 12.9-$\sigma$ significant acceleration of the primary with 2 degrees of freedom \citep[][]{BrandtHGCA2021}). \textbf{The statistically significant acceleration of HIP 5319 is suggestive of the presence of a previously unseen low-mass companion. Therefore we chose to observe this target in an attempt to uncover any previously unimaged low-mass companions around this accelerating star, following a similar method of target selection as in \citet{Currie2020} and \citet{Steiger2021}.}


==> oldtext.tex <==

--old

Over the past two decades direct imaging detections of exoplanets around young, nearby stars have increased with facility adaptive optics (AO) systems and now extreme adaptive optics systems \citep{Marois2008, Marois2010, Kuzuhara2013, Currie2015, Macintosh2015,Chauvin2017,Keppler2018,Currie2022a}.
%(\citet{Marois2008, Marois2010}, \citet{Kuzuhara2013}, \citet{Currie2013, Currie2015, Currie2020}, \citet{Macintosh2015}, \citet{Chauvin2017}, \citet{Keppler2018}). 
The majority of these detections have been of companions at separations greater than $\rho\sim0\farcs{}4$ and correspond to separations of 10-150 au from their host stars \citep[][]{Nielsen2019,Vigan2021,Currie2022b}. 

More recently, second generation extreme AO systems such as the Subaru Coronagraphic Extreme Adaptive Optics system \citep[SCExAO;][]{Jovanovich2015b, Ahn2021} and the Magellan Extreme Adaptive Optics system \citep[MagAO-X;][]{Males2020} have enabled deeper contrasts at separations less than $\rho\lesssim0\farcs{}4$. These deeper contrasts - in conjunction with noise-reducing techniques such as Stochastic Speckle Discrimination \citep[SSD;][]{Walter2019} and Angular, Spectral, and Reference Differential Imaging \citep[ADI, SDI, RDI;][]{Marois2006, Marois2000, Ruane2019} - have led to the discovery of companions with orbital radii less than 10 au \citep[][]{Chilcote2021, Steiger2021}. By continuing to drive to deeper contrasts at narrower separations we will be able to directly image companions with orbits closer to their host stars and around host stars at greater distances from earth.

%The challenges of reaching sufficient contrasts to image young, bright exoplanets is one of the chief reasons for the low yield of blind direct imaging surveys.
\textbf{The low occurrence rates of planets which can be detected via direct imaging at contrasts achievable by current instruments and extreme AO systems} is one of the chief reasons for the low yield of blind direct imaging surveys. Fortunately the \textit{Hipparcos-Gaia Catalog of Accelerations} \citep[HGCA;][]{BrandtHGCA2021} combines absolute astrometry from the Hipparcos and \textit{Gaia} missions \citep[][]{GaiaMission}, which allows a more targeted search of nearby stars that have astrometric accelerations that suggest the presence of yet-undiscovered companions. Direct imaging surveys that target these stars with significant astrometric acceleration have already yielded discoveries of companions on solar-system scales and have also enabled a better ability to characterize them (\citet{Calissendorff2018, Fontanive2019, Currie2020, Currie2021, Bowler2021, Chilcote2021, Steiger2021, Brandt2019, Brandt2021, Kuzuhara2022,Currie2022c}). \citep{Currie2022c}

\textcolor{red}{As astrometry-selected direct imaging programs become more prevalent so too will the discovery of previously undetected, uncharacterized companions. When characterizing the planets, one may use code such as \texttt{orvara} \citep[][]{Brandt2021} to fit for orbital parameters of the system such as the masses of the primary star and any existing companions as well as the eccentricity, semimajor axis, and inclination of the companion's orbit. In cases with significant coverage of a companion's orbit, archival radial velocity, astrometry for the primary, or a combination of the three, the user may be able to use the out-of-the-box priors from dynamical orbit fitting codes and achieve accurate estimates of the orbital parameters of the system without digging into the underlying assumptions used by the code. However, for systems which have not been frequently targeted and do not have archival data as such the data may not be extremely constraining for determining the parameters of system. In this paper we explore how different assumptions that go into fitting for system parameters may affect the interpretation of the results which may be as significant as the characterization of a substellar companion as a low-mass star or vise versa.}

Here we report the direct imaging discovery of HIP 5319 B, a low mass, candidate substellar companion around the F-type star HIP 5319 A using SCExAO coupled with the MKID Exoplanet Camera \citep[MEC;][]{Walter2020}, the Visible Aperture Masking Polarimetric Imager for Resolved Exoplanetary Structures \citep[VAMPIRES;][]{Norris2015}, the Coronagraphic High Angular Resolution Imaging Spectrograph \citep[CHARIS;][]{Groff2016}, and the NIRC2 camera on Keck. 


---


HIP 5319 ($^{\star}$78 Psc) is an F5IV spectral class star \citep{BoroSaikia2018} at $d=$42.93$\pm$0.06 pc (\citet{GaiaMission}, \citet{GaiaDR2}).

% The \textit{Hipparcos-Gaia} Catalog of Accelerations reports a $\chi^{2}=$171.04: evidence of a 12.9-$\sigma$ significant acceleration of the primary with 2 degrees of freedom \citep[][]{BrandtHGCA2021}). \textbf{The statistically significant acceleration of HIP 5319 is suggestive of the presence of a previously unseen low-mass companion. Therefore we chose to observe this target in an attempt to uncover any previously unimaged low-mass companions around this accelerating star, following a similar method of target selection as in \citet{Currie2020} and \citet{Steiger2021}.}

It has previously been identified as an RS CVn binary star by \citet{Fleming1989}, who measured a projected rotation rate of \textit{v}sin(\textit{i})=68$\pm$20.5 km/s and x-ray luminosity of $L_{x}=9.2\pm3.7\times10^{28}$ erg/s. RS CVn binaries typically have \textbf{orbital} periods less than 14 days, show high levels of chromospheric activity \textbf{via strong emission in Calcium II H and K lines, and have a hotter component of spectral type F or G \citep[][]{Montesinos1988}}. Both variation in the reported rotation rate and high chromospheric activity have been reported for this star, the latter via \textbf{Ca II} H $\&$ K lines \citet{BoroSaikia2018} measured log($R^\prime_{HK}$)= $-$4.016\textbf{, which tracks the strength of the emission at the cores of the 2 lines}. Multiple sources have reported \textit{v}sin(\textit{i}) values with significant scatter: 125 km/s \citep[][]{Danziger1972}, 68$\pm$20.5 km/s \citep[][]{Fleming1989}, 36.4$\pm$4.8 km/s \citep[][]{deMedeiros1999}, 35 km/s \citep[][]{Nordstrom2004}, and 41.5 km/s (\citet{Glebocki2005}, \citet{Glebocki2005Catalog}).

\textcolor{red}{The extreme chromospheric activity measured by \citet{BoroSaikia2018} is evidence for the extreme youth of HIP 5319. The chromospheric index of log($R^\prime_{HK}$)=-4.016 easily exceeds chromospheric activity values from stars in the Pleiades and Hyades associations and is comparable or higher to the stars in the Scorpius-Centaurus (Sco-Cen) association \citep[][]{MamajekHillenbrand2008, Pecaut2013}. Its Hertzsprung-Russel diagram position in \textit{Gaia} color-magnitude space ($M_{G}$ vs $G_{BP}-G_{RP}$=2.97, 0.54) lies between the Pleiades and Hyades, which is consistent with either a main sequence star between 115 and $\sim$800 Myr or a pre-main sequence star much younger than the Pleiades.}

In contrast to this characterization of HIP 5319 as a \textcolor{red}{young,} short period binary, the Gaia Early Data Release 3 \citep[Gaia eDR3;][]{GaiaEDR3} reports that HIP 5319 is well fit by a 5-parameter single star solution whose Renormalized Unit Weight Error (RUWE) is 1.01, \textbf{ruling out most stellar companions with a period between of P$\lesssim$10 days}.
%(Timothy Brandt, private communication).

\textcolor{red}{The fractional X-ray luminosity of the star is log($L_{x}$/$L_{bol}$)$\sim$-4.9, almost two orders of magnitude less than a typical pre-main sequence star, which would have values log($R^\prime_{HK}$)$\sim$-4.0 and log($L_{x}$/$L_{bol}$)$\sim$-3.2 for the chromospheric activity and fractional X-ray luminosity, respectively. This mix of chromospheric and coronal activity is therefore atypical compared to other young, active stars. The star also does not appear to be near any other stars or known associations that are $\lesssim$100 Myr. Several authors have estimate the age of the star using isochrones and have found values of $1.6^{+0.3}_{-0.4}$ Gyr \citep[][]{Holmberg2009} and 1.07-1.23 Gyr using Padova and BASTI models \citep[][]{Casagrande2011}, lending credence to its identification as an older, single star.}

\textcolor{red}{Ultimately, the two conflicting identifications of the HIP 5319 primary as either a young, chromospherically active binary or an older single star that lacks Calcium II HK emission will have significant implication on the understanding of the stellar system and interpretation of any of its companions' properties. If there is not significant HK emission and little evidence of binarity then the higher age estimate is likely the correct one, which will anchor the interpretation of its companion.} In addition to performing a direct imaging search for such a binary companion, a spectroscopic \textbf{study} of the primary with a high resolution spectrograph is necessary to disentangle the possible identities of the star and settle on the correct interpretation. This will be discussed further in sections \ref{sub:primary_single_star} and \ref{sub:ca_hk}.

More recently, HIP 5319 was observed by the Transiting Exoplanet Survey Satellite \citep[TESS;][]{TESS_Mission} and has 2-minute cadence photometry for one sector. This observation may be too short to show spots reliably, but it does show pulsations with a period of just less than 1 day\footnote{Accessed via \url{https://mast.stsci.edu/portal/Mashup/Clients/Mast/Portal.html}}. It was also observed once by the International Ultraviolet Explorer (IUE) during IUE Program ID: CB401 \citep[Stellar Chromospheres;][]{Blanco1982}. In the spectrum from IUE\footnote{Accessed via \url{https://archive.stsci.edu/iue/obtaining.html}}, HIP 5319 A shows strong emission from the Lyman $\alpha$ line. These two data points show signs that the primary might be chromospherically active, though follow up observation is required to determine the nature of this activity.

The \textit{Hipparcos-Gaia} Catalog of Accelerations reports a $\chi^{2}=$171.04: evidence of a 12.9-$\sigma$ significant acceleration of the primary with 2 degrees of freedom \citep[][]{BrandtHGCA2021}). \textbf{The statistically significant acceleration of HIP 5319 is suggestive of the presence of a previously unseen low-mass companion. Therefore we chose to observe this target in an attempt to uncover any previously unimaged low-mass companions around this accelerating star, following a similar method of target selection as in \citet{Currie2020} and \citet{Steiger2021}.}

